Optimizing Neural Networks through Activation Function Discovery and Automatic Weight Initialization

Automated machine learning (AutoML) methods improve upon existing models by optimizing various aspects of their design. While present methods focus on hyperparameters and neural network topologies, other aspects of neural network design can be optimized as well. To further the state of the art in AutoML, this dissertation introduces techniques for discovering more powerful activation functions and establishing more robust weight initialization for neural networks. These contributions improve performance, but also provide new perspectives on neural network optimization. First, the dissertation demonstrates that discovering solutions specialized to specific architectures and tasks gives better performance than reusing general approaches. Second, it shows that jointly optimizing different components of neural networks is synergistic, and results in better performance than optimizing individual components alone. Third, it demonstrates that learned representations are easier to optimize than hard-coded ones, creating further opportunities for AutoML. The dissertation thus makes concrete progress towards fully automatic machine learning in the future.

==> chapters/aquasurf/sections/abstract.tex <==
\begin{abstract}

Carefully designed activation functions can improve the performance of neural networks in many machine learning tasks.  However, it is difficult for humans to construct optimal activation functions, and current activation function search algorithms are prohibitively expensive.  This paper aims to improve the state of the art through three steps: First, the benchmark datasets \texttt{Act-Bench-CNN}, \texttt{Act-Bench-ResNet}, and \texttt{Act-Bench-ViT} were created by training convolutional, residual, and vision transformer architectures from scratch with 2{,}913 systematically generated activation functions. Second, a characterization of the benchmark space was developed, leading to a new surrogate-based method for optimization. More specifically, the spectrum of the Fisher information matrix associated with the model's predictive distribution at initialization and the activation function's output distribution were found to be highly predictive of performance. Third, the surrogate was used to discover improved activation functions in CIFAR-100 and ImageNet tasks.  Each of these steps is a contribution in its own right; together they serve as a practical and theoretical foundation for further research on activation function optimization.  Code is available at \codeurl, and the benchmark datasets are at \dataurl.
    
\end{abstract}


==> chapters/aquasurf/sections/compute_infrastructure.tex <==
\section{Compute Infrastructure}
\label{sec:aquasurf:compute_infrastructure}

The experiments in this paper were implemented using an AWS \texttt{g5.48xlarge} instance with eight NVIDIA A10G GPUs.  The total compute cost for the search experiments in Section \ref{sec:aquasurf:search_new_tasks} was 14.49 GPU-hours for All-CNN-C on CIFAR-100, 21.67 GPU-hours for ResNet-56 on CIFAR-100, and 196.25 GPU-days for MobileViTv2-0.5 on ImageNet.  This cost includes the time to train the eight baseline activation functions and then to evaluate 100 additional functions.  The instance ran in Oregon (\texttt{us-west-2}) and was powered by renewable energy, so the experiments for this paper contributed no carbon emissions.


==> chapters/aquasurf/sections/experiment_details.tex <==
\section{Experiment Details}
\label{sec:aquasurf:experiment_details}

This section specifies the details for the experiments in Chapter \ref{chap:aquasurf}. Several variations to the approach presented in the main text were also evaluated in preliminary experiments. The approach turned out to be robust to most of them, but the results also justify the choices used for the main experiments.

\paragraph{Training Details}
\input{chapters/aquasurf/figures/training_details.tex}
For CIFAR-10 and CIFAR-100, balanced validation sets were created by sampling 5{,}000 images from the training set.  Full training details and hyperparameters are listed in Table \ref{tab:aquasurf:training_details}.


\paragraph{Search Implementation}
In order to predict performance for an unevaluated activation function, the function outputs and FIM eigenvalues must first be computed.  Thus, the searches in Section \ref{sec:aquasurf:search_new_tasks} were implemented in three steps.  First, activation function outputs for all 425,896 activation functions in the search space were calculated.  This computation is inexpensive and easily parallelizable.  Second, eight workers operated in parallel to sample activation functions uniformly at random from the search space and calculate their FIM eigenvalues.  Third, once the number of activation functions with FIM eigenvalues calculated reached 5{,}000, seven of the workers began the search by evaluating the functions with the highest predicted performance.  The eighth worker continued calculating FIM eigenvalues for new functions so that their performance could be predicted during the search. This setup allowed taking best advantage of the available compute for the regression-type search methods.

The experiments on ImageNet required substantially more compute than the experiments on CIFAR-100.  For this reason, all eight workers evaluated activation functions once the number of functions with FIM eigenvalues reached 7{,}000.

Computing FIM eigenvalues took approximately 26 seconds, 84 seconds, and 37 seconds per activation function for All-CNN-C, ResNet-56, and MobileViTv2-0.5, respectively.  This cost is not trivial, but it is well worth it, as the experiments in Chapter \ref{chap:aquasurf} show.


\paragraph{Unique Activation Functions}
Different computation graphs can result in the same activation function (e.g.\ $\max\{x,0\}$ and $\max\{0,x\}$).  In the benchmark dataset and in the larger search space of Section \ref{sec:aquasurf:search_new_tasks}, repeated activation functions were filtered out.  1{,}000 inputs were sampled $\mathcal{N}(0,1)$ and truncated to $[-5,5]$.  Two activation functions were considered the same if their outputs were identical.

\input{chapters/aquasurf/figures/fim_default_n_neighbors.tex}
\paragraph{Improving the Combined UMAP Projection}
Figure \ref{fig:aquasurf:fim_default_n_neighbors} displays a projection of FIM eigenvalues using default UMAP hyperparameters.  The plots show the eigenvalues organized in multiple distinct one-dimensional manifolds.  Again, FIM eigenvalues are noisy features; there are some clusters of activation functions achieving similar performance, but there are also regions where performance varies widely.  As mentioned in the main text, this issue was addressed by reducing the UMAP parameter \texttt{n\_neighbors} to 3.  This change reduced the connectivity of the low-dimensional FIM eigenvalue representation, resulting in a space with many distinct clusters (as seen in Figure \ref{fig:aquasurf:umap_embeddings}).  

On its own, this setting did not improve the search on the benchmark datasets.  However, it did improve performance when the FIM eigenvalues were combined with activation function outputs (as was discussed in Section \ref{sec:aquasurf:visualizing_umap}).  The reason is that the UMAP model for the activation function outputs did not decrease \texttt{n\_neighbors}, and so the combined UMAP model relied more on the activation function outputs than it did on the FIM eigenvalues.  As Figure \ref{fig:aquasurf:umap_embeddings} shows, the activation function outputs are reliable but sometimes project good activation functions to distinct regions in the search space.  Introducing extra connectivity into the fuzzy topological representation via the FIM eigenvalues was sufficient to address this issue, bringing good activation functions to common regions of the space.


\paragraph{Increasing the Dimension of the UMAP Projections}
The UMAP plots show two-dimensional projections of FIM eigenvalues and activation function outputs.  Regression algorithms were also trained on five and 10-dimensional projections.  These runs resulted in comparable or worse performance. Therefore, the two-dimensional projections were selected for simplicity and for consistency between the algorithm implementation and figure visualizations.


\paragraph{Gaussian Process Regression}
As an alternative search method, Gaussian process regression (GPR) was evaluated in activation function search. Several different acquisition mechanisms were used, including expected improvement, probability of improvement, maximum predicted value, and upper confidence bound.  The approach worked well, but the results were inconsistent across the different acquisition mechanisms.  GPR was also more expensive to run compared to the algorithms in the main text (KNR, RFR, SVR), and so those algorithms were used instead for simplicity and efficiency.

\paragraph{Adjusting $k$ in KNR}
The initial experiments with the KNR algorithm used $k=3$.  Experimenting with $k=\{1,5,8\}$ did not reliably improve performance, so $k=3$ was kept.


\paragraph{Uniformly Spaced Inputs for Activation Function Outputs}
In an alternative implementation, equally spaced inputs from $-5$ to $5$ were given to the activation functions instead of normally distributed inputs. This variation did not noticeably change the quality of the embeddings nor the performance of the search algorithms. Therefore, normal inputs were used for consistency with Equation \ref{eq:aquasurf:dist_fn_outputs}.  Figure \ref{fig:aquasurf:interpolation} is the only exception; it used 80 inputs equally spaced from $-5$ to $5$ and increased the UMAP parameter \texttt{min\_dist} to 0.5.  These settings improved the quality of the reconstructed activation functions in the plot.


==> chapters/aquasurf/sections/introduction.tex <==
\section{Introduction}
\label{sec:aquasurf:introduction}

Activation functions are an important choice in neural network design \cite{apicella2021survey, nwankpa2018activation}.  In order to realize the benefits of good activation functions, researchers often design new functions based on characteristics like smoothness, groundedness, monotonicity, and limit behavior.  While these properties have proven useful, humans are ultimately limited by design biases and by the relatively small number of functions they can consider.  On the other hand, automated search methods can evaluate thousands of unique functions, and as a result, often discover better activation functions than those designed by humans.  However, such approaches do not usually have a theoretical justification, and instead focus only on performance.  This limitation results in computationally inefficient ad hoc algorithms that may miss good solutions and may not scale to large models and datasets.

This paper addresses these drawbacks in a data-driven way through three steps. First, in order to provide a foundation for theory and algorithm development, convolutional, residual, and vision transformer based architectures were trained from scratch with 2{,}913 different activation functions, resulting in three activation function benchmark datasets: \texttt{Act-Bench-CNN}, \texttt{Act-Bench-ResNet}, and \texttt{Act-Bench-ViT}.  These datasets make it possible to analyze activation function properties at a large scale in order to determine which are most predictive of performance.

The second step was to characterize the activation functions in these benchmark datasets analytically, leading to a surrogate performance measure. Exploratory data analysis revealed two activation function properties that are highly indicative of performance: (1) the spectrum of the Fisher information matrix associated with the model’s predictive distribution at initialization, and (2) the activation function’s output distribution.  Both sets of features contribute unique information.  They are both predictive of performance on their own, but they are most powerful when used in tandem.  These features were combined to create a metric space where a low-dimensional representation of the activation functions could be learned. This space can then be used as a surrogate in the search for good activation functions.

In the third step, this surrogate was evaluated experimentally, first by verifying that it can discover known good functions in the benchmark datasets efficiently and reliably, and second by demonstrating that it can discover improved activation functions in new tasks on CIFAR-100 and ImageNet. The representation turned out to be so powerful that an out-of-the-box regression algorithm was able to search it effectively.  The approach, called \technique (\techniqueexpanded), is orders of magnitude more efficient than past work.  Indeed, whereas previous approaches evaluated hundreds or thousands of activation functions, \technique requires only tens of evaluations in order to discover functions that outperform a wide range of baseline activation functions in each context.  Code implementing the \technique algorithm is available at \codeurl.

Prior research on activation function optimization and Fisher information matrices is reviewed in Section~\ref{sec:related_work}. This work extends it in three ways. First, the benchmark collections are made available at \dataurl, providing a foundation for further research on activation function optimization.  Second, the low-dimensional representation of the Fisher information matrix makes it a practical surrogate measure, making it possible to apply it to not only activation function design, but potentially also to other applications in the future. Third, the already-discovered functions can be used immediately to improve performance in image processing tasks, and potentially in other tasks in the future. 

==> chapters/aquasurf/sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

The techniques in this paper were inspired by prior research in multiple areas, including neural architecture and activation function search, as well as research on the FIM.

\paragraph{Neural Architecture Search}
In neural architecture search \citep[NAS;][]{wistuba2019survey, elsken2019neural, zoph2016neural}, the goal is to design a neural network architecture automatically.  NAS approaches typically focus on optimizing the type and location of the layers and the connections between them, but often use standard activation functions like ReLU.  This work in complimentary to NAS approaches, because it uses standard architectures but optimizes the design of the activation function.

\paragraph{Zero-cost NAS Proxies}
Recently, zero-cost NAS proxies have received increased attention \cite{white2021powerful, shen2021proxybo, mellor2020neural}.  These approaches aim to accelerate neural architecture search by using cheap surrogate calculations in place of expensive full training of architectures.  This paper adopts a similar approach, using FIM eigenvalues and activation function outputs to predict which activation functions are likely to be most promising before dedicating resources to evaluating them.  

\paragraph{Activation Function Search}
Methods for automatically discovering activation functions include reinforcement learning \cite{DBLP:conf/iclr/RamachandranZL18}, evolutionary computation \cite{bingham2020gecco, bingham2022discovering, liu2020evolving, basirat2018quest}, and gradient-based methods \cite{apl-agostinelli2014learning, pade-molina2019pad, goyal1906learning, tavakoli2020splash, bingham2022discovering}.  This paper builds upon existing work, focusing on efficient search and on understanding the properties that make activation functions effective.

\paragraph{Other Uses of the FIM}
This paper used FIM eigenvalues to predict the performance of different activation functions.  The FIM is an important quantity in machine learning with several uses.  One important example is optimal experiment design \cite{emery1998optimal}, where experiments are designed to be optimal with respect some criterion.  The criteria vary, but are often functions of the eigenvalues of the FIM, such as the maximum or minimum eigenvalue, or the trace of the FIM (sum of the eigenvalues) or determinant of the FIM (product of the eigenvalues).  Instead of choosing one optimality criterion and only considering one summary statistic, this paper keeps all of the eigenvalues of the FIM and learns an optimal distribution experimentally.  

Past work has also used the eigenvalues of the FIM to determine suitable values of the batch size or learning rate for neural networks \cite{liao2018approximate, hayase2021spectrum, karakida2021pathological, furusho2019effects, furusho2020theoretical}. The FIM provides insights to the learning dynamics of SGD \cite{jastrzebski2021catastrophic} and the dynamics of signal propagation at different layers in networks with and without batch normalization layers \cite{huang2020layer}.  The FIM has also been used to develop second-order optimization algorithms for neural networks \cite{grosse2016kronecker, martens2015optimizing, martens2018kronecker}. Applying it to activation function design is thus a compelling further opportunity.


==> chapters/aquasurf/sections/search_space.tex <==
\section{Activation Function Search Spaces}
\label{sec:aquasurf:search_space}
\input{chapters/aquasurf/figures/search_space.tex}

The activation functions in this chapter were implemented as computation graphs from the PANGAEA search space \cite{bingham2022discovering}. The space includes unary and binary operators, in addition to existing activation functions \cite{nair2010rectified, elu, selu, DBLP:conf/iclr/RamachandranZL18, elfwing2018sigmoid}. This approach allows specifying families of functions in a compact manner. It is thus possible to focus the search on a space where good functions are likely to be located, and also to search it comprehensively.

\paragraph{Benchmark Datasets}
The benchmark datasets introduced in Section \ref{sec:aquasurf:activation_function_datasets} contain every activation function of the three-node form \texttt{binary(unary($x$),unary($x$))} using the operators in Table \ref{tab:aquasurf:search_space}.  The result is 5{,}103 activation functions, of which 2{,}913 are unique. This space is visualized in Figure~\ref{fig:aquasurf:umap_embeddings}.  

For \texttt{Act-Bench-CNN} and \texttt{Act-Bench-ResNet}, the accuracies are the median from three runs.  For \texttt{Act-Bench-ViT}, the results are from single runs due to computational costs.

\paragraph{New Tasks}
The experiments in Section \ref{sec:aquasurf:search_new_tasks} utilized a larger search space.  Specifically, it was based on the following four-node computation graphs: 
\texttt{binary(unary(unary($x$)),unary($x$))},
\texttt{binary(unary($x$),unary(unary($x$)))},
\texttt{n-ary(unary($x$),unary($x$),unary($x$))},
\texttt{unary(binary(unary($x$),unary($x$)))}, and
\texttt{unary(unary(unary(unary($x$))))}.
The unary and binary nodes used the operators in Table \ref{tab:aquasurf:search_space}, and the $n$-ary node used the sum, product, maximum, and minimum operators.  Together, these computation graphs create a search space with 1{,}023{,}516 functions, of which 425{,}896 are unique. This space is visualized in Figure~\ref{fig:aquasurf:large_search_space}.



==> chapters/autoinit/figures/afn_plots.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{chapters/autoinit/plots/afn_plots.pdf}\\[2em]
    \includegraphics[width=\linewidth]{chapters/autoinit/plots/zero_gaussian_mean_afn_plots.pdf}
 \caption{A representative sample of top-performing activation functions from the PANGAEA search space.  Each plot is titled with the function definition and the accuracy achieved when paired with All-CNN-C initialized with AutoInit or AutoInit++.  Some activation functions are fixed, while others have learnable parameters $\alpha$, $\beta$, and $\gamma$.  AutoInit is compatible with both types of functions.  For the parametric ones, the red line shows the activation function at initialization, with $\alpha = \beta = \gamma = 1$.  The blue lines show the shapes the activation function takes during training, created by sampling values for the learnable parameters from $\mathcal{U}(0.5, 2.0)$.  By achieving good performance with all of these functions, AutoInit demonstrates flexibility that should turn out useful for developing new activation functions in the future.}
    \label{fig:autoinit:afn_plots}
\end{figure}
% functional duplicates removed


==> chapters/autoinit/figures/allcnnc_activation_fn.tex <==
\begin{table}
    \centering
    \begin{tabular}{lll}
        \toprule
        Activation & Glorot Uniform & AutoInit \\ 
        \midrule
        ELU & 89.53 & 89.69 {\color{ForestGreen} \scriptsize (+0.16)} \\
        GELU & 89.81 & 89.90 {\color{ForestGreen} \scriptsize (+0.09)} \\
        ReLU & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
        SELU & 90.06 & 90.02 {\color{OrangeRed} \scriptsize (-0.04)} \\
        Softplus & 10.00 & 87.83 {\color{ForestGreen} \scriptsize (+77.83)} \\
        Softsign & 52.60 & 59.59 {\color{ForestGreen} \scriptsize (+6.99)} \\
        Swish & 89.67 & 89.46 {\color{OrangeRed} \scriptsize (-0.21)} \\
        tanh & 71.28 & 73.36 {\color{ForestGreen} \scriptsize (+2.08)} \\
        \bottomrule
    \end{tabular}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different activation functions and weight initialization strategies.  Results are shown as the median of three independent runs.  AutoInit stabilizes training by adapting to each activation function.}
    \label{tab:autoinit:allcnnc_activation_fn}
\end{table}

==> chapters/autoinit/figures/allcnnc_dropout.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         Dropout Rate & Default Init & AutoInit \\ 
%         \midrule
%         0.0 (no dropout) & 89.13 & 89.68 {\color{ForestGreen} \scriptsize (+0.55)} \\
%         0.1 & 88.51 & 90.22 {\color{ForestGreen} \scriptsize (+1.71)} \\
%         0.2 & 88.91 & 89.76 {\color{ForestGreen} \scriptsize (+0.85)} \\
%         0.3 & 89.45 & 89.77 {\color{ForestGreen} \scriptsize (+0.32)} \\
%         0.4 & 88.25 & 89.93 {\color{ForestGreen} \scriptsize (+1.68)} \\
%         0.5 (default setting) & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         0.6 & 87.28 & 89.99 {\color{ForestGreen} \scriptsize (+2.71)} \\
%         0.7 & 88.61 & 89.50 {\color{ForestGreen} \scriptsize (+0.89)} \\
%         0.8 & 86.55 & 88.95 {\color{ForestGreen} \scriptsize (+2.40)} \\
%         0.9 & 84.41 & 85.64 {\color{ForestGreen} \scriptsize (+1.23)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_dropout}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{chapters/autoinit/plots/allcnnc_dropout.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different dropout rates and weight initialization strategies.  Each result is from a single run.  AutoInit improves accuracy in every case and gets good performance with a wider range of dropout values compared to the default initialization.}
    \label{fig:autoinit:allcnnc_dropout}
\end{figure}

==> chapters/autoinit/figures/allcnnc_l2_penalty.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         L2 Penalty & Default Init & AutoInit \\ 
%         \midrule
%         0 & 88.93 & 90.20 {\color{ForestGreen} \scriptsize (+1.27)} \\
%         0.00001 & 91.91 & 92.25 {\color{ForestGreen} \scriptsize (+0.34)} \\
%         0.0001 & 92.17 & 92.67 {\color{ForestGreen} \scriptsize (+0.50)} \\
%         0.001 (default) & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         0.01 & 10.00 & 47.91 {\color{ForestGreen} \scriptsize (+37.91)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_l2_penalty}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{chapters/autoinit/plots/allcnnc_l2_penalty.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different weight decay settings and weight initialization strategies.  Each result is from a single run.  AutoInit outperforms the default strategy in every case.}
    \label{fig:autoinit:allcnnc_l2_penalty}
\end{figure}


==> chapters/autoinit/figures/allcnnc_lr_scale.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         LR Scale & Default Init & AutoInit \\ 
%         \midrule
%         0.1 & 78.57 & 85.06 {\color{ForestGreen} \scriptsize (+6.49)} \\
%         0.2 & 83.78 & 87.21 {\color{ForestGreen} \scriptsize (+3.43)} \\
%         0.5 & 85.53 & 89.39 {\color{ForestGreen} \scriptsize (+3.86)} \\
%         1 & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         2 & 90.15 & 90.13 {\color{OrangeRed} \scriptsize (-0.02)} \\
%         5 & 89.31 & 89.24 {\color{OrangeRed} \scriptsize (-0.07)} \\
%         10 & 11.22 & 15.36 {\color{ForestGreen} \scriptsize (+4.14)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_lr_scale}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{chapters/autoinit/plots/allcnnc_lr_multiplier.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different learning rate schedule multipliers and weight initialization strategies.  Each result is from a single run.  AutoInit is comparable to or outperforms the default initialization strategy in every case.  AutoInit also achieves good performance with a broader range of learning rate schedules compared to the default strategy.}
    \label{fig:autoinit:allcnnc_lr_scale}
\end{figure}

==> chapters/autoinit/figures/codeepneat.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{chapters/autoinit/plots/codeepneat.pdf}
    \caption{The CoDeepNEAT method.  Modules (middle) replace the nodes in the blueprint (left) to create a candidate neural network (right).  CoDeepNEAT produces a variety of network architectures, which then provide a comprehensive evaluation of the generality of AutoInit.}
    % \caption{The CoDeepNEAT method for coevolving populations of modules and blueprints.  The modules (middle) replace the nodes in the blueprint (left) to create a candidate neural network (right).  Each module species is evolved separately, and each node in the blueprint specifies the species from which the module is drawn to replace it. CoDeepNEAT produces a variety of network architectures, which then provide a comprehensive evaluation of the generality of AutoInit.}
    \label{fig:autoinit:codeepneat}
\end{figure}

==> chapters/autoinit/figures/evolved_models.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.33\linewidth]{chapters/autoinit/network_visualizations/mnist.pdf} \\
    \textbf{MNIST} \\[2em]
    \includegraphics[width=0.33\linewidth]{chapters/autoinit/network_visualizations/pmlb.pdf} \\
    \textbf{PMLB Adult} \\[2em]
    \includegraphics[width=0.33\linewidth]{chapters/autoinit/network_visualizations/textclassifier.pdf} \\
    \textbf{Wikipedia Toxicity}
    \caption{Three representative networks evolved with AutoInit for the MNIST, PMLB Adult, and Wikipedia Toxicity tasks.  Although the networks are distinctly different from current models in the literature, AutoInit is able to initialize them properly, leading to good performance in each case. }
    \label{fig:autoinit:evolved_models}
\end{figure*}



==> chapters/autoinit/figures/pangaea.tex <==

\usetikzlibrary{shapes.geometric, arrows, positioning, calc}
\tikzstyle{input} = [rectangle, rounded corners, text centered, draw=black, fill=red!30]
\tikzstyle{unary} = [rectangle, rounded corners, text centered, draw=black, fill=yellow!30]
\tikzstyle{binary} = [rectangle, rounded corners, text centered, draw=black, fill=blue!30]
\tikzstyle{arrow} = [thick, ->,>=stealth]
\tikzstyle{output} = [rectangle, rounded corners, text centered, draw=black, fill=green!30]
\tikzstyle{invisible} = [rectangle, text centered]
\tikzstyle{maybeparam} = [draw, circle, dashed, fill=cyan!30]

\begin{figure*}
    \centering
    \begin{adjustbox}{max width=\linewidth}
        {\renewcommand{\arraystretch}{2}%
        \begin{tabular}{c@{\hskip 3em}c@{\hskip 3em}c@{\hskip 3em}c}
            {\renewcommand{\arraystretch}{1}%
            \begin{tabular}{llll} 
                \toprule 
                \multicolumn{3}{c}{\textbf{Unary}} & \multicolumn{1}{l}{\textbf{Binary}} \\ \midrule
                $0$                & $e^x-1$               & $\textrm{ReLU}(x)$        & $x_1 + x_2$ \\
                $1$                & $\log(\sigma(x))$     & $\textrm{ELU}(x)$         & $x_1 - x_2$ \\
                $x$                & $\textrm{erf}(x)$     & $\textrm{SELU}(x)$        & $x_1 \cdot x_2$ \\
                $-x$               & $\textrm{erfc}(x)$    & $\textrm{Swish}(x)$       & $x_1 / x_2$ \\
                $|x|$              & $\textrm{sinh}(x)$    & $\textrm{Softplus}(x)$    & $x_1^{x_2}$ \\
                $x^{-1}$           & $\textrm{cosh}(x)$    & $\textrm{Softsign}(x)$    & $\max\{x_1, x_2\}$ \\
                $x^2$              & $\textrm{tanh}(x)$    & $\textrm{HardSigmoid}(x)$ & $\min\{x_1, x_2\}$\\
                $e^x$              & $\textrm{arcsinh}(x)$ & $\textrm{bessel\_i0e}(x)$ & \\
                $\sigma(x)$        & $\textrm{arctan}(x)$  & $\textrm{bessel\_i1e}(x)$ & \\

                
                \bottomrule
            \end{tabular}}

            &
            
            \begin{tikzpicture}[node distance=3em, baseline=-4.5em]
            
                \node (output2) [output] {$f(x)$};
                \node (unary4) [unary, below of=output2] {Unary};
                \node (unary3) [unary, below of=unary4] {Unary};
                \node (input3) [input, below of=unary3] {$x$};
                
                \draw [arrow] (input3) -- (unary3);
                \draw [arrow] (unary3) -- (unary4);
                \draw [arrow] (unary4) -- (output2);
            
                \node (output) [output, right of=output2, xshift=4em] {$f(x)$};
                \node (binary) [binary, below of=output] {Binary};
                \node (unary1) [unary, below of=binary, xshift=-2em] {Unary};
                \node (unary2) [unary, below of=binary, xshift=2em] {Unary};
                \node (input1) [input, below of=unary1] {$x$};
                \node (input2) [input, below of=unary2] {$x$};
                
                \draw [arrow] (input1) -- (unary1);
                \draw [arrow] (input2) -- (unary2);
                \draw [arrow] (unary1) -- (binary);
                \draw [arrow] (unary2) -- (binary);
                \draw [arrow] (binary) -- (output);

            \end{tikzpicture}
            &
            \begin{tabular}{cccccccc}
     
                \begin{tikzpicture}[node distance=3em]
        
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1] (b1) {$x_1 + x_2$};
                    \node [unary, below of=b1, xshift=-2em] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Parent};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1] (b1) {$x_1 + x_2$};
                    \node [unary, below of=b1, xshift=-2em, draw=red, line width=1] (swish) {$\textrm{Swish}(x)$};
                    \node [unary, below of=swish] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Insert};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (swish);
                    \draw [arrow] (swish) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [unary, below of=u1] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Remove};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow, draw=red] (u3) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1, draw=red, line width=1] (b1) {$x_1 \cdot x_2$};
                    \node [unary, below of=b1, xshift=-2em] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Change};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1, draw=red, line width=1] (u1) {$-x$};
                    \node [binary, below of=u1, draw=red, line width=1] (b1) {$\max\{x_1, x_2\}$};
                    \node [unary, below of=b1, xshift=-2em, draw=red, line width=1] (u2) {$0$};
                    \node [unary, below of=b1, xshift=2em, draw=red, line width=1] (u3) {$\textrm{tanh}(x)$};
                    \node [unary, below of=u3, draw=red, line width=1] (u4) {$\textrm{SELU}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Regenerate};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
            \end{tabular}
            &
            \begin{tabular}{cc}            
                \begin{tikzpicture}[node distance=3em]
                
                    \node (output) [output] {$f(x)$};
                    \node (unary) [unary, below of=output] {$\sigma(x)$};
                    \node (binary) [binary, below of=unary] {$x_1 - x_2$};
                    \node (unary1) [unary, below of=binary, xshift=-2em] {$|x|$};
                    \node (unary2) [unary, below of=binary, xshift=2em] {$\textrm{arctan}(x)$};
                    \node (input1) [input, below of=unary1] {$x$};
                    \node (input2) [input, below of=unary2] {$x$};
            
                    \draw [arrow] (input1) -- (unary1);
                    \draw [arrow, draw=red] (input2) -- (unary2);
                    \draw [arrow, draw=red] (unary1) -- (binary);
                    \draw [arrow] (unary2) -- (binary);
                    \draw [arrow] (binary) -- (unary);
                    \draw [arrow, draw=red] (unary) -- (output);
                    
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
        
                    \node (output) [output] {$f(x)$};
                    \node (p1) [maybeparam, below of=output] {$\alpha$};
                    \node (unary) [unary, below of=p1] {$\sigma(x)$};
                    \node (binary) [binary, below of=unary] {$x_1 - x_2$};
                    \node (p5) [maybeparam, below of=binary, xshift=-2em] {$\beta$};
                    \node (unary1) [unary, below of=p5] {$|x|$};
                    \node (unary2) [unary, below of=binary, xshift=2em] {$\textrm{arctan}(x)$};
                    \node (p4) [maybeparam, below of=unary2] {$\gamma$};
                    \node (input1) [input, below of=unary1] {$x$};
                    \node (input2) [input, below of=p4] {$x$};
                    
            
                    \draw [arrow] (input1) -- (unary1);
                    \draw [arrow] (input2) -- (p4);
                    \draw [arrow] (p4) -- (unary2); 
                    \draw [arrow] (unary1) -- (p5);
                    \draw [arrow] (p5) -- (binary);
                    \draw [arrow] (unary2) -- (binary);
                    \draw [arrow] (binary) -- (unary);
                    \draw [arrow] (unary) -- (p1);
                    \draw [arrow] (p1) -- (output);
                    
                \end{tikzpicture}
            \end{tabular}
            \\
            {\LARGE \textbf{(a) Search Space}}
            &
            {\LARGE \textbf{(b) Initialization}}
            &
            {\LARGE \textbf{(c) Mutation}}
            &
            {\LARGE \textbf{(d) Parameterization}}
            
        \end{tabular}}
    \end{adjustbox}
    \caption{The PANGAEA method \cite{bingham2020discovering} for representing activation functions.  (a) \textbf{Search Space:} Activation functions are represented as computation graphs composed of unary and binary operators.   (b) \textbf{Initialization: }A randomly created activation function has one of two possible functional forms: either $f(x) = \texttt{unary1}(\texttt{unary2}(x))$ or $f(x) = \texttt{binary}(\texttt{unary1}(x), \texttt{unary2}(x))$.   (c) \textbf{Mutation:} Randomly selected mutations modify the original parent activation function.   (d) \textbf{Parameterization:} Up to three learnable parameters are added to the activation function in order to allow the function's shape to be fine-tuned via gradient descent.  For example, the rightmost computation graph represents the parametric activation function $f(x) = \alpha \cdot \sigma (\beta \cdot | x | - \arctan ( \gamma \cdot x ) )$. In this manner, PANGAEA generates a variety of activation functions that can be used to evaluate AutoInit's generality and flexibility.}
    \label{fig:autoinit:pangaea}
\end{figure*}


==> chapters/autoinit/figures/resnet_vary_lr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{chapters/autoinit/plots/resnet_vary_lr.pdf}
    \includegraphics[width=0.49\linewidth]{chapters/autoinit/plots/resnet_vary_lr_no_bn.pdf}
    \caption{ResNet-164 test accuracy on CIFAR-10 with a variety of learning rate schedules and weight initializations.  Results are from a single run.  AutoInit is comparable to or outperforms the default initialization in every case.}
    \label{fig:autoinit:resnet_vary_lr}
\end{figure}

==> chapters/autoinit/figures/signal_propagation_afn.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{chapters/autoinit/plots/signal_propagation_vary_afn.pdf}
    \caption{Signal propagation across All-CNN-C networks with different activation functions.  Gaussian input was propagated through the networks and the empirical variance computed at each layer.  The variance naturally fluctuates as each layer modifies its input.  At layers with weights (highlighted in red), AutoInit scales the weights appropriately to return the variance to approximately 1.0.}
    \label{fig:autoinit:signal_propagation_afn}
\end{figure}

==> chapters/autoinit/figures/signal_propagation_dropout.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{chapters/autoinit/plots/signal_propagation_vary_dropout.pdf}
    % \includegraphics[width=0.49\linewidth]{plots/signal_propagation_vary_dropout_default.pdf}
    % \includegraphics[width=0.49\linewidth]{plots/signal_propagation_vary_dropout_autoinit.pdf}
    \caption{Signal propagation in All-CNN-C networks with different dropout rates.  The plots were created by feeding Gaussian inputs to the network and computing the empirical variance at each layer.  GAP2D refers to a \texttt{GlobalAveragePooling2D} layer. With the default initialization, signal variance vanishes with depth, and the behavior is different with each dropout rate.  With AutoInit, the signal variance remains approximately constant at 1.0 after each layer with initializable weights (highlighted in red).  The variance is consistent across the network regardless of the dropout rate.}
    \label{fig:autoinit:signal_propagation_dropout}
\end{figure}

==> chapters/autoinit/figures/usage.tex <==
\begin{figure}
    \centering
    \begin{verbatim}
        # Install
        pip install git+https://github.com/~~~ANONYMIZED~~~/
        
        # Import
        from autoinit.initializer.initalize_weights import AutoInit
        
        # Initialize
        model = AutoInit().initialize_model(model)
    \end{verbatim}
    \caption{The AutoInit package provides a wrapper around TensorFlow models.}
    \label{fig:autoinit:usage}
\end{figure}

% TODO
% Update code with latest ENN changes
% Change name from universal to autoinit


==> chapters/autoinit/sections/appendices.tex <==
\section*{Appendices}
The following appendices can be found online at \url{https://arxiv.org/abs/2109.08958}.
\begin{itemize}
    \item[A:] Mean and Variance Estimation for Different Layer Types
    \item[B:] Convolutional, Residual, and Transformer Network Experiment Details
    \item[C:] Neural Architecture Search Experiment Details
    \item[D:] Statistical Significance of Results in Activation Function Meta-Learning
    \item[E:] Future Work
    \item[F:] Computing Infrastructure
\end{itemize}
In particular, Appendix \ref{sec:mean_variance_estimation} contains mean and variance mapping functions $g$ for the following layer types:


{\small
\noindent\textbf{Weights } \texttt{Conv\{1D,2D,3D\}}, \texttt{DepthwiseConv\{1D,2D\}}, \texttt{Dense}

\noindent\textbf{Activation Functions } \texttt{Activation}, \texttt{elu}, \texttt{expo\-nen\-tial}, \texttt{gelu}, \texttt{hard\_sigmoid}, \texttt{LeakyReLU}, \texttt{linear}, \texttt{PReLU}, \texttt{ReLU}, \texttt{selu}, \texttt{sigmoid}, \texttt{softplus}, \texttt{softsign}, \texttt{swish}, \texttt{tanh}, \texttt{ThresholdedReLU}

\noindent\textbf{Dropout } \texttt{SpatialDropout\{1D,2D,3D\}}, \texttt{Dropout}

\noindent\textbf{Pooling } \texttt{AveragePooling\{1D,2D,3D\}}, \texttt{MaxPooling\{1D,\allowbreak2D,3D\}},  \texttt{Global\-Average\-Pooling\{1D,2D,3D\}}, \texttt{Glo\-bal\-Max\-Pooling\{1D,2D,3D\}}

\noindent\textbf{Normalization } \texttt{BatchNormalization}, \texttt{GroupNorma\-li\-za\-tion}, \texttt{LayerNormalization}

\noindent\textbf{Arithmetic } \texttt{Add}, \texttt{Average}, \texttt{Subtract}, \texttt{Multiply}, \texttt{tf.mat\-mul}, \texttt{tf.reduce\_mean}, \texttt{tf.reduce\_sum}

\noindent\textbf{Recurrent } \texttt{GRU}, \texttt{LSTM}, \texttt{SimpleRNN}

\noindent\textbf{Shape Adjustment } \texttt{Flatten}, \texttt{Permute}, \texttt{Reshape}, \texttt{Up\-Sampling\{1D,2D,3D\}}, \texttt{Cropping\{1D,2D,3D\}}, \texttt{tf.re\-shape}, \texttt{tf.split}, \texttt{tf.transpose}

\noindent\textbf{Misc. } \texttt{Concatenate}, \texttt{ZeroPadding\{1D,2D,3D\}}, \texttt{Input\-Layer}
}

==> chapters/autoinit/sections/computing_infrastructure.tex <==
\section{Computing Infrastructure}
\label{sec:autoinit:compute_infrastructure}
Experiments in this paper were run in a distributed framework using StudioML software \cite{gorunner, StudioML} to place jobs on machines with NVIDIA GeForce GTX 1080 Ti and RTX 2080 Ti GPUs.  The CoAtNet experiments (Section \ref{sec:autoinit:coatnet}) were run on an AWS g5.48xlarge instance with NVIDIA A10G GPUs.  Training CoAtNet on Imagenette required an average of 0.91 GPU hours per run.  Training CoAtNet on ImageNet once took 119.89 GPU hours.  Training on Imagenette instead of ImageNet therefore emit approximately $119.89 / 0.91 \approx 132$ times less carbon.  The AutoInit package is available at \url{https://github.com/cognizant-ai-labs/autoinit}.


==> chapters/autoinit/sections/discussion.tex <==
% % this section was not used, the future_work file was used instead
% \section{Discussion}
% % \label{sec:discussion} 

% autoinit suggests new default hyperparameter values --> this suggests the old parameters were compensating for incorrect init

% should accelerate model development in the future

% doesn't have to be the total optimal in every case, but it is a solid default setting that has good motivation behind it

% Batchnorm has some good properties, some bad properties.  AutoInit may help to ease the transition away from using bn since it is compatible in both cases.

==> chapters/autoinit/sections/domain_details.tex <==
\section{Experiment domain details}
\label{sec:experiment_domain_details}

% This section describes the experimental setups for each domain in greater detail.

% \subsection{MNIST}

% Models evolved for MNIST were trained for five epochs using the Adam optimizer and batch size 128 \cite{kingma2014adam}.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  No data augmentation was applied to the images.



% \subsection{Omniglot}

% Models were trained for three epochs during evolution, with 1000 iterations per epoch.  No data augmentation is applied to the images.  The initial learning rate is an evolved hyperparamter chosen on a log scale between 0.0001 and 0.001.  


% The learning rate then decays as $\texttt{learning\_rate} = 0.1^{\texttt{epoch}/10}*\texttt{initial\_learning\_rate}$ during training.



% \subsection{PMLB (Adult)}

% The evolved models are trained for 25 epochs with the Adam optimizer \cite{kingma2014adam}.  The batch size is 32.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  No data augmentation was used.
%https://github.com/EpistasisLab/pmlb/blob/master/datasets/adult/metadata.yaml


% \subsection{Wikipedia Toxicity}

% The models are trained with the Adam optimizer \cite{kingma2014adam} for three epochs with a batch size of 128.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  Input tokens are capped at a maximum sentence length of 220.


% \subsection{Oxford 102 Flower}

% The model is optimized with stochastic gradient descent with Nesterov momentum 0.9.  The learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.1.  Another evolved hyperparameter, \texttt{weight\_decay\_to\_lr\_ratio}, is evolved on a log scale between $10^{-7}$ and $10^{-3}$, and then weight decay (as an L2 loss) of $\texttt{weight\_decay\_to\_lr\_ratio} * \texttt{learning\_rate}$ is applied to all weights and biases.  During training, a batch size of 8 is used, and training progresses for 30 epochs.

% Images are augmented to improve generalization performance.  Images are randomly flipped horizontally, are rotated up to 40 degrees, shifted up/down and left/right up to 20\%, and shear intensity and zoom range are both up to 20\%.

% To save compute resources, training ends early if validation accuracy does not improve for ten consecutive epochs.

% \subsection{ChestX-ray14}

% The ChestX-ray14 dataset contains 112,120 high resolution RGB frontal chest X-ray images \cite{wang2017chestx}.  For each image, the task is to identify the presence or absence of 14 different diseases: some X-rays can have multiple diseases, while others are disease-free.  This dataset naturally lends itself to a multitask learning setup, where there are 14 binary classification tasks associated with each iamge.  The dataset is divided into a 70\%/10\%20\% training/validation/testing split.  The metric used to evaluate networks is the average area under the ROC curve for all 14 tasks (AUROC).  Because many approaches in this task use ImageNet pretrained models, a common preprocessing step which is used here is to resize all images to be 224x224 \cite{deng2009imagenet, wang2017chestx}.

% Models are trained for four epochs.  The models are optimized with Adam \cite{kingma2014adam}.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.001, and it decreases by a factor of 0.1 if the validation loss has not improved for three epochs.  The learning rate decreases in this way at most two times during training.  


% The batch size is one.  The number of training samples is reduced to 20,000 to speed up training.  These samples are randomly selected by stratified sampling.  Let the ratio of positive and negative samples in the dataset be $r_p$ and $r_n$, respectively.  Positive samples are sampled at a rate of $e^{r_p / 0.6} / (e^{r_p / 0.6} + e^{r_n / 0.6})$ while negative samples are sampled at a rate of $e^{r_n / 0.6} / (e^{r_p / 0.6} + e^{r_n / 0.6})$.  This induces a minor bias towards a slightly more balanced dataset, without entirely abandoning the original data distribution.



==> chapters/autoinit/sections/enn_details.tex <==
\section{Neural Architecture Search Experiment Details}
\label{sec:autoinit:enn_details}

\input{chapters/autoinit/figures/enn_results_detail.tex}


This appendix contains implementation details for the experiments in Section \ref{sec:autoinit:nas}.  The progress of CoDeepNEAT in these experiments was shown in Figure \ref{fig:autoinit:enn_results} in the main text.  Figure \ref{fig:autoinit:enn_results_detail} shows this same data but in greater detail.  Table \ref{tab:autoinit:hyperparameters} contains the training hyperparameters, neural network layers, evolutionary hyperparameters, and mutation probabilities used in each of the five tasks.  The five tasks used with CoDeepNEAT are:

\input{chapters/autoinit/figures/hyperparameters.tex}

\paragraph{Vision} The MNIST dataset contains 28x28 grayscale images of handwritten digits 0-9.  There are 60,000 training images (5,000 of which were used for validation) and 10,000 test images \cite{lecun2010mnist}.  MNIST is used under the Creative Commons Attribution-Share Alike 3.0 license.

\paragraph{Language} In the Wikipedia Toxicity dataset, the task is to classify English Wikipedia comments as toxic or healthy contributions \cite{wulczyn2017ex}.  The dataset contains 92,835, 31,227, and 30,953 comments in the training, validation, and test sets, respectively.  

\paragraph{Tabular} In the Adult dataset \cite{kohavi1996scaling} from the Penn Machine Learning Benchmarks repository \citep[PMLB;][]{Olson2017PMLB}) the task is to predict whether an individual makes over \$50K per year based on 14 features.  Out of 48,842 total instances, 20\% are randomly separated to create a test set.  The dataset is used under the MIT License.

\paragraph{Multi-Task} The Omniglot dataset contains handwritten characters in 50 different alphabets \cite{lake2015human}; classifying characters in each alphabet is a natural multi-task problem.  The characters are $105 \times 105$ grayscale images, and there are 20 instances of each character.  To save compute resources, 20 of the 50 alphabets were randomly selected for experiments.  A fixed training, validation, and testing split of 50\%, 20\%, and 30\% was used with each task.  The learning rate decays as $\texttt{learning\_rate} = 0.1^{\texttt{epoch}/10}*\texttt{initial\_learning\_rate}$ during training.  The dataset is used under the MIT License.

\paragraph{Transfer Learning} A DenseNet-121 network is first pretrained on the ImageNet dataset \cite{deng2009imagenet, huang2017densely}. Models are then evolved to utilize its embeddings to classify images in the Oxford 102 Flower dataset, consisting of 102 types of flowers found in the United Kingdom \cite{Nilsback08}.  Each class has between 40 and 258 images; the training and validation sets have 10 images per class, and the test set contains the remaining images from the dataset.  During training, the weight decay (L2 loss) is scaled by the current learning rate.  Images are also augmented to improve generalization performance.  Images are randomly flipped horizontally, rotated up to 40 degrees, shifted up/down and left/right up to 20\%, and shear intensity and zoom range varied up to 20\%.




==> chapters/autoinit/sections/evolved_models.tex <==
\section{Evolved models}
\label{sec:evolved_models}


This section includes visualizations of models evolved for different tasks.  The visualizations illustrate the flexibility of AutoInit.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/mnist.pdf}
%     \caption{MNIST}
%     \label{fig:mnist}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[height=0.95\textheight]{network_visualizations/omniglot.pdf}
%     \caption{Omniglot}
%     \label{fig:omniglot}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/pmlb.pdf}
%     \caption{PMLB (Adult)}
%     \label{fig:pmlb}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/textclassifier.pdf}
%     \caption{Wikipedia Toxicity}
%     \label{fig:textclassifier}
% \end{figure}




==> chapters/autoinit/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Proper weight initialization is crucial to achieve high performance with deep networks.  A common motif in such networks is repeated layers or building blocks.  Thus, if a given layer amplifies or diminishes the forward or backward propagation of signals, repeated applications of that layer will result in exploding or vanishing signals, respectively \cite{hochreiter1991untersuchungen, hanin2018neural}.  This phenomenon makes optimization difficult, and can even exceed machine precision. The issue persists regardless of whether the weights are sampled to be uniform, normal, or orthogonal \cite{saxe2013exact, hu2020provable}.

While many initialization strategies have been proposed in the past, these strategies apply only to neural networks with specific activation functions, topologies, or layer types.  Thus, researchers designing new models or activation functions have two options.  The first option is to derive weight initialization strategies manually for every architecture considered, which is generally difficult and time consuming.  The second option is to use existing initialization strategies in new settings, where they may be incorrect and therefore misleading:  A candidate model may appear poor when it is the suboptimal initialization that makes training difficult.

To overcome this problem, this paper proposes AutoInit, an algorithm that automatically calculates analytic mean- and variance-preserving weight initialization for neural networks.  Since AutoInit is algorithmic, it relieves the researcher from a difficult but consequential step in model design.  It is no longer necessary to use existing weight initialization strategies in incorrect settings: AutoInit provides an appropriate default initialization automatically, resulting in better and more reliable performance.

%% SHORTER VERSION
% The remainder of this paper reviews existing work in weight initialization (\S \ref{sec:related_work}), describes the AutoInit algorithm (\S \ref{sec:algorithm}), presents experiments showing the power and generality of AutoInit (\S \ref{sec:experiments}) and discusses plans for AutoInit in the future (\S \ref{sec:future_work}).

%% LONGER VERSION
% The remainder of this paper is organized as follows.  Section \ref{sec:related_work} reviews existing work in weight initialization.  It shows how current initialization methods impose constraints such as requiring a specific activation function or network structure.  Section \ref{sec:algorithm} details the high-level algorithm for AutoInit, and presents the analytic mean and variance calculations for signals as they propagate through each type of layer.  Section \ref{sec:experiments} presents experiments demonstrating that AutoInit is robust and improves performance across a range of neural networks, data modalities, hyperparameter settings, and task scenarios.  The results show that AutoInit is well-equipped to initialize existing models and likely models that have yet to be discovered.  Section \ref{sec:future_work} details plans for AutoInit in the future, including variations on the AutoInit algorithm, support for new layer types, tighter deep learning framework integration, and experiments in reinforcement learning, generative, and other domains.



==> chapters/autoinit/sections/related_work.tex <==

\section{Related Work}
\label{sec:related_work}

Weight initialization strategies attempt to solve the following fundamental problem: How should weights be initialized so that the neural network does not suffer from vanishing or exploding signals? This section briefly reviews research in this area,
with a more extensive survey in Appendix \ref{ap:related_work_extended}.

Many early contributions stabilized signal propagation in feedforward and convolutional networks, but only when used with specific activation functions \cite{glorot2010understanding, lecun2012efficient, he2015delving}.  After the introduction of residual networks \citep[ResNets;][]{he2016deep, he2016identity}, new weight initialization schemes were developed to account for shortcut connections and various types of residual branches, but these approaches similarly imposed design constraints like requiring specific block structures and activation functions \cite{taki2017deep, zhang2019fixup, arpit2019initialize}.  Data-dependent weight initializations rely on empirical variance estimates derived from the data in order to be model-agnostic \cite{krahenbuhl2015data}.  However, these approaches introduce a computational overhead \cite{mishkin2015all} and suffer when the network is very deep \cite{zhang2019fixup}.

Thus, previous techniques solved the initialization problem for networks with specific activation functions, topologies, and layer types. In contrast, AutoInit does not impose design constraints or incur a parameter overhead \cite{dauphin2019metainit, zhu2021gradinit} and is therefore a good starting point especially in new settings. 





==> chapters/autoinit/sections/related_work_extended.tex <==
\section{Related Work}
\label{sec:related_work_extended}

Weight initialization strategies attempt to solve the following problem: How should weights be initialized so that the neural network does not suffer from vanishing or exploding signals?  This section reviews previous research in neural network weight initialization, which has focused on stabilizing signals by accounting for specific components of neural networks such as the activation function, topology, layer types, and training data distribution.


\paragraph{Activation-Function-Dependent Initialization}
\label{sec:weight_init_for_afns}
As is common in the literature, \texttt{fan\_in} and \texttt{fan\_out} refer to the number of connections feeding into and out of a node, respectively.  \citet{lecun2012efficient} recommend sampling weights from a distribution with mean zero and standard deviation $\sqrt{\texttt{fan\_in}}$.  This initialization encourages propagated signals to have variance approximately one if used with an activation function symmetric about the origin, like $1.7159\tanh\left(\frac{2}{3}x\right)$ or $\tanh(x) + \alpha x$ for some small choice of $\alpha$. The standard sigmoid $f(x) = 1/(1+e^{-x})$ induces a mean shift and should not be used in this setting.

\citet{glorot2010understanding} proposed one initialization strategy to ensure unit variance in the forward-propagated signals and another to ensure unit variance for the backward-propagated gradients.  As a compromise between the two strategies, they initialized weights by sampling from $\mathcal{U}\left(-\frac{\sqrt{6}}{\sqrt{\texttt{fan\_in} + \texttt{fan\_out}}}, \frac{\sqrt{6}}{\sqrt{\texttt{fan\_in} + \texttt{fan\_out}}}\right)$.  They also avoided sigmoid, and instead chose symmetric functions with unit derivatives at 0, such as tanh or Softsign$(x) = x/(1+|x|)$.

\citet{he2015delving} introduced the PReLU activation function and a variance-preserving weight initialization to be used with it that samples weights from $\mathcal{N}(0, \sqrt{2/\texttt{fan\_in}})$.  Similarly, \citet{selu} introduced SELU, an activation function with self-normalizing properties.  These properties are only realized when SELU is used with the initialization scheme by \citet{lecun2012efficient}.

The above weight initialization strategies attempt to solve the same fundamental problem: How can weights be scaled so that repeated applications of the activation function do not result in vanishing or exploding signals?  While these approaches solve this problem in a few special cases, the issue is more general.  Manually deriving the correct scaling is intractable for complicated activation functions.  One approach for an arbitrary function $f$ is to sample Gaussian inputs $x$ and adjust the weights according to the empirical variance $\textrm{Var}(f(x))$ \cite{brock2021characterizing}.  This paper proposes an alternative and potentially more accurate approach: integration by adaptive quadrature.  The result is a weight initialization strategy that is compatible with any integrable activation function.  Indeed, previous activation-function-dependent initializations are special cases of the AutoInit algorithm.


\paragraph{Topology-Dependent Initialization}
The activation-function-dependent initializations discussed above were designed for neural networks composed of convolutional or dense layers.  After the introduction of residual networks \citep[ResNets;][]{he2016deep, he2016identity}, new weight initialization schemes had to be developed to account for the effect of shortcut connections and various types of residual branches.

\citet{taki2017deep} analyzed signal propagation in plain and batch-normalized ResNets.  They developed a new weight initialization to stabilize training, but did not consider modifications like using deeper residual blocks or reordering components like the activation function or batch normalization layers.  In contrast, AutoInit is topology-agnostic: It adapts to any of these changes automatically.

\citet{zhang2019fixup} introduced Fixup, an initialization method that rescales residual branches to stabilize training.  Fixup replaces batch normalization in standard and wide residual networks \cite{ioffe2015batch, he2016deep, he2016identity, zagoruyko2016wide} and replaces layer normalization \cite{ba2016layer} in transformer models \cite{vaswani2017attention}.  The disadvantages of this scheme are that it only applies to residual architectures, needs proper regularization to get optimal performance, and requires additional learnable scalars that slightly increase model size.

\citet{arpit2019initialize} proposed a new initialization scheme for weight-normalized networks \cite{salimans2016weight} that relies on carefully scaling weights, residual blocks, and stages in the network.  Like related approaches, this technique improves performance in specific cases, but imposes design constraints, like requiring ReLU activation functions and a specific Conv $\rightarrow$ ReLU $\rightarrow$ Conv block structure.

Just as tanh-inspired weight initialization does not stabilize training of ReLU networks, initialization schemes designed for non-residual networks fail with ResNets \cite{hanin2018start, bachlechner2020rezero, brock2021characterizing}.
This observation suggests that future classes of neural networks will again require developing new weight initializations.  Additionally, practitioners with models that do not fit neatly within the restricted settings of existing weight initialization research are left to derive their own initialization or use a suboptimal one.  For example, many initialization schemes assume that the activation function is ReLU \cite{he2015delving, taki2017deep, arpit2019initialize, zhang2019fixup, de2020batch}.  Indeed, ReLU is currently the most popular activation function \cite{nwankpa2018activation, apicella2021survey}, but it is not the best choice in every case.  ReLU prevents dynamical isometry \cite{saxe2013exact, pennington2017resurrecting}, weakens adversarial training \cite{xie2020smooth}, and results in poorer accuracy compared to other activation functions in certain tasks \cite{bingham2022discovering}.  A general weight initialization strategy that does not impose architectural constraints and achieves good performance in diverse settings is needed. AutoInit is designed to meet this challenge.



\paragraph{Layer-Dependent Initialization}
\citet{hendrycks2016adjusting} noted that dropout layers \cite{srivastava2014dropout} also affect the variance of forward-propagated signals in a network.  To stabilize training properly, it is necessary to take dropout layers and the specific dropout rate into account in weight initialization.  In fact, pooling, normalization, recurrent, padding, concatenation, and other layer types affect the signal variance in a similar way, but current initialization schemes do not take this effect into account.  AutoInit is designed to adapt to each of these layer types dynamically, and can be extended to include new layer types as they are introduced in the future.

\paragraph{Data-Dependent Initialization}
\citet{mishkin2015all} fed data samples through a network and normalized the output of each layer to have unit variance.  \citet{krahenbuhl2015data} adopted a similar approach, but opted to normalize along the channel dimension instead of across an entire layer.  Data-dependent weight initializations are most similar in spirit to AutoInit; they rely on empirical variance estimates derived from the data in order to be model-agnostic.  However, data-dependent weight initializations introduce a computational overhead \cite{mishkin2015all}, and are not applicable in settings where data is not available or its distribution may shift over time, such as online learning or reinforcement learning.  The quality of the initialization is also dependent on the number of the data samples chosen, and suffers when the network is very deep \cite{zhang2019fixup}.  AutoInit instead uses an analytic approach for greater efficiency and higher accuracy.

\paragraph{Summary}
Thus, previous techniques solved the initialization problem for networks with specific activation functions, topologies, and layer types. In contrast, AutoInit does not impose design constraints, depend on data samples, or incur a parameter overhead \cite{dauphin2019metainit, zhu2021gradinit} and is therefore a good starting point especially in new settings. 




==> chapters/autoinit/sections/training_details.tex <==
\section{Convolutional, Residual, and Transformer Network Experiment Details}
\label{sec:autoinit:training_details}

This Section contains implementation details for the experiments in Sections \ref{sec:autoinit:convolutional}-\ref{sec:autoinit:autoinit_vs_lsuv}.

\paragraph{All-CNN-C} The training setup follows that of \citet{springenberg2015striving} as closely as possible.  The network is trained with SGD and momentum 0.9.  The dropout rate is 0.5 and weight decay as L2 regularization is 0.001.  The data augmentation involves featurewise centering and normalizing, random horizontal flips, and random $32 \times 32$ crops of images padded with five pixels on all sides.  The initial learning rate is 0.01 and is decreased by a factor of 0.1 after epochs 200, 250, and 300 until training ends at epoch 350.

Because \citet{springenberg2015striving} did not specify how they initialized their weights, the networks are initialized with the ``Glorot Uniform'' strategy \citep[also called Xavier initialization; ][]{glorot2010understanding}, where weights are sampled from $\mathcal{U}\left(-\frac{\sqrt{6}}{\sqrt{\texttt{fan\_in} + \texttt{fan\_out}}}, \frac{\sqrt{6}}{\sqrt{\texttt{fan\_in} + \texttt{fan\_out}}}\right)$. This initialization is the default setting in TensorFlow,\footnote{\url{https://github.com/tensorflow/tensorflow/blob/v2.5.0/tensorflow/python/keras/layers/convolutional.py\#L608-L609}} and is sufficient to replicate the results reported by \citet{springenberg2015striving}. 

\paragraph{Residual Networks}
The networks are optimized with SGD and momentum 0.9.  Dropout is not used, and weight decay is 0.0001.  Data augmentation includes a random horizontal flip and random $32 \times 32$ crops of images padded with four pixels on all sides.  



\paragraph{CoAtNet}

A smaller variant of the CoAtNet architecture\footnote{\url{https://github.com/leondgarse/keras_cv_attention_models/blob/v1.3.0/keras_cv_attention_models/coatnet/coatnet.py\#L199}} was used in order to fit the model and data on the available GPU memory.  The architecture has three convolutional blocks with 64 channels, four convolutional blocks with 128 channels, six transformer blocks with 256 channels, and three transformer blocks with 512 channels.  This architecture is slightly deeper but thinner than the original CoAtNet-0 architecture, which has two convolutional blocks with 96 channels, three convolutional blocks with 192 channels, five transformer blocks with 384 channels, and two transformer blocks with 768 channels \cite{dai2021coatnet}.  The models are otherwise identical.

The training hyperparameters were inspired by \citet{wightman2021resnet} and are common in the literature.  Specifically, images were resized to $160 \times 160$.  The learning rate schedule was increased linearly from $1e^{-4}$ to $4e^{-4}$ for six epochs and it then followed a cosine decay until epoch 105.  Weight decay was set to 0.02 times the current learning rate at each epoch.  The model was trained with batch size 256 and optimized with AdamW \cite{loshchilov2017decoupled_adamw}.  Data augmentation included RandAugment applied twice with a magnitude of six \cite{cubuk2020randaugment}.  Mixup and Cutmix were also used with alpha 0.1 and 1.0, respectively \cite{zhang2017mixup, yun2019cutmix}.  The training images were augmented with random resized crops \cite{szegedy2015going} that were at minimum 8\% of the original image; after training the model was evaluated on 95\% center crops.

As discussed in Section \ref{sec:autoinit:mean_variance_estimation}, AutoInit maintains signal variance $\nu=1$, but it is also possible to adjust $\nu$ if desired.  In the CoAtNet experiments, $\nu = 0.01$ was found to give the best performance among $\nu = \{1, 0.1, 0.01, 0.001\}$.  The experiment removing normalization layers used the default of $\nu = 1$.

\paragraph{ImageNet} The experiment in Section \ref{sec:autoinit:imagenet} used the same training setup as the experiments with CoAtNet on Imagenette in the previous paragraph except for two changes.  The batch size was 2{,}048 (512 per GPU across four GPUs), and the maximum learning rate was $3.2e^{-2}$.

\paragraph{Data-Dependent Initialization Comparison}
In the experiments in Section \ref{sec:autoinit:autoinit_vs_lsuv}, a learning rate schedule inspired by superconvergence \cite{smith2019super} was used to save time.  The learning rate increases linearly to 0.1 during the first five epochs, and then decreases linearly for 20 epochs, after which training ends.  The weight decay for All-CNN-C was also decreased by a factor of 10.  This modification is common when networks are trained with superconvergence \cite{smith2019super}.


\paragraph{Initialization Time}
It is important to note that AutoInit does not incur a significant overhead.  Each layer must be visited once to be initialized, so the complexity is $O(L)$ where $L$ is the number of layers.  For example: All-CNN-C, ResNet-56, and ResNet-164 take 1, 33, and 106 seconds to initialize.  The costs are hardware-dependent, but only spent once, and are small compared to the cost of training.



==> chapters/gecco/figures/cnn.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{chapters/gecco/images/cnn.png}
    \caption{Convolutional neural network used in preliminary experiments.  This simple architecture trains quickly, allowing for fast experimentation, while still achieving good results.}
    \label{fig:gecco:cnn}
\end{figure}

==> chapters/gecco/figures/histogram.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{chapters/gecco/images/mnist_hist.pdf}
    \includegraphics[width=0.85\linewidth]{chapters/gecco/images/cifar_hist.pdf}
    \caption{Histogram of MLP and CNN accuracies on the MNIST and CIFAR-10 datasets when trained with different activation functions.  Accuracy with ReLU \cite{nair2010rectified}, $\sigma(x) = (1+e^{-x})^{-1}$, $\textrm{Swish}(x) = x \cdot \sigma(x)$ \cite{DBLP:conf/iclr/RamachandranZL18, elfwing2018sigmoid}, and $\textrm{tanh}(x)$ are shown with vertical lines.  There exist many activation functions that outperform all of these baseline functions, verifying that activation function search is a promising research direction.}
    \label{fig:gecco:histogram}
\end{figure}

==> chapters/gecco/sections/introduction.tex <==
\section{Introduction}
\label{sec:gecco:introduction}

Together with topology, loss function, and learning rate, the choice of activation function plays a large role in determining how a neural network learns and behaves.  
An activation can be any arbitrary function that transforms the output of a layer in a neural network.
However, only a small number of activation functions are widely used in modern deep learning architectures. 
The Rectified Linear Unit, $\textrm{ReLU}(x) = \max\{x, 0\}$, is popular because it is simple and effective.  Other activation functions such as $\textrm{tanh}(x)$ and $\sigma(x) = 1 / (1 + e^{-x})$ are commonly used when it is useful to restrict the activation value within a certain range.  There have also been attempts to engineer new activation functions to have certain properties.  For example, Leaky ReLU \cite{maas2013rectifier} allows information to flow when $x < 0$.  Softplus \cite{nair2010rectified} is positive, monotonic, and smooth.  Many hand-engineered activation functions exist \cite{nwankpa2018activation}, but none have achieved widespread adoption comparable to ReLU.  Activation function design can therefore be seen as a largely untapped resource in neural network design.
  
This situation points to an interesting opportunity: it may be possible to optimize activation functions automatically through metalearning.  Rather than attempting to directly optimize a single model as in traditional machine learning, metalearning seeks to find better performance over a space of models, such as a collection of network architectures, hyperparameters, learning rates, or loss functions~\cite{finn2017model, finn2017meta, elsken2019neural, wistuba2019survey, feurer2015initializing, gonzalez2019improved}.  Several techniques for metalearning have been proposed, including gradient descent, Bayesian hyperparameter optimization, reinforcement learning, and evolutionary algorithms \cite{chen2019progressive, feurer2015initializing, zoph2016neural, real2019regularized}.  Of these, evolution is the most versatile and can be applied to several aspects of neural network design.

This work develops an evolutionary approach to optimize activation functions.  Activation functions are represented as trees, and novel activation functions are discovered through crossover, mutation, and exhaustive search in expressive search spaces containing billions of candidate activation functions.  The resulting functions are unlikely to be discovered manually, yet they perform well, surpassing traditional activation functions like ReLU on image classification tasks CIFAR-10 and CIFAR-100.

This paper continues with Section \ref{sec:related_work}, which presents a summary of related research in metalearning and neural network optimization, and discusses how this work furthers the field. Section \ref{sec:evolution} explains how activation functions are evolved in detail, defining the search space of candidate functions as well as the implementation of crossover and mutation.  In Section \ref{sec:experiments}, a number of search strategies are presented, and results of the experiments are given in Section \ref{sec:results}.  This work continues with discussion and potential future work in Section \ref{sec:discussion}, before concluding in Section \ref{sec:conclusion}.
  
  

==> chapters/pangaea/figures/changing_size.tex <==
\begin{figure*}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \includegraphics[width=0.33\linewidth]{images/width.pdf}
    \includegraphics[width=0.33\linewidth]{images/depth.pdf}
    \includegraphics[width=0.33\linewidth]{images/resnetv2.pdf}
    \end{adjustbox}
    \caption{CIFAR-100 test accuracy for different neural networks and activation functions.  Accuracy with ReLU is shown in blue, and accuracy with the specialized activation functions in red.  The relative improvement of the specialized functions over ReLU is shown as a dotted green line, according to the axis values on the right of each plot.  \textbf{Left:} The depth of Wide ResNet is fixed at 10, and the width varies from 1 to 16.  \textbf{Center:} The depth of Wide ResNet varies from 10 to 34, while the width is fixed at four.  \textbf{Right:} The depth of Preactivation ResNet ranges from 20 to 164.  The width and depth of a network can affect how much a specialized activation function outperforms ReLU.}
    \label{fig:pangaea:changing_size}
\end{figure*}



==> chapters/pangaea/figures/instability.tex <==
\begin{figure}
    \centering
    \begin{multicols}{3}
    82.90\% Accuracy
    \includegraphics[clip, trim=0em 0em 0em 2.25em, width=\linewidth]{chapters/pangaea/images/83pct.png}\\
    75.36\% Accuracy
    \includegraphics[clip, trim=0em 0em 0em 2.25em, width=\linewidth]{chapters/pangaea/images/75pct.png}\\
    53.46\% Accuracy\\
    \includegraphics[clip, trim=0em 0em 0em 2.25em, width=\linewidth]{chapters/pangaea/images/53pct.png}
    \end{multicols}
    \caption{Three identical training runs (different random seeds) with the activation function $\cos(x) \cdot \sigma(x)$ produce very different final accuracies.  When the preactivation distribution stays to the left of the peak at $x=0$, accuracy is high.  The farther across the peak the early layer's preactivation distribution shifts, the poorer the accuracy becomes.  The plots show that the periodic nature of the activation function caused training to be unstable.  Thus, periodic operators such as $\sin(x)$ and $\cos(x)$ were removed from the search space for experiments in Chapter \ref{chap:pangaea} (Table \ref{tab:pangaea:searchspace}).}
    \label{fig:pangaea:instability}
\end{figure}

==> chapters/pangaea/figures/moving_acc_runtime.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/moving_acc.pdf}
    % Maybe we don't need this one.  What's the point it is making anyway?
    % \includegraphics[width=0.49\linewidth]{images/moving_runtime.pdf}
    \caption{Average population fitness across time for two independent PANGAEA processes.  The plots show the average validation accuracy achieved with the $P=64$ most recently evaluated activation functions at any given time in the search process.  The two PANGAEA runs behave similarly, gradually discovering better activation functions as they explore the search space.}
    \label{fig:pangaea:moving_acc_runtime}
\end{figure}

==> chapters/pangaea/figures/preactivation.tex <==
\begin{figure}[t]
    \centering
    \begin{multicols}{3}
    \includegraphics[width=\linewidth]{chapters/pangaea/images/epoch5.png}\\
    \includegraphics[width=\linewidth]{chapters/pangaea/images/epoch40.png}\\
    \includegraphics[width=\linewidth]{chapters/pangaea/images/epoch95.png}
    \end{multicols}
    \caption{Preactivation distribution for the $\sigma(x) \cdot \textrm{erf}(x)$ activation function (shown as a red line) when used with the CNN of Figure \ref{fig:gecco:cnn} at training epochs 5, 40, and 95.  The early layer preactivation distribution (shown in green) corresponds to the distribution of values in the network immediately before the first activation function is applied, while the late layer preactivation (shown in purple) is the distribution of values immediately before the final activation function in the network is applied.  The graphics were created by computing a histogram of the early and late layer preactivation distributions, and then overlaying these histograms on the plot of activation function itself.  Thus, areas where the activation function appears thick represent parts of the activation function that are heavily utilized by the neural network, while areas where the activation function appears thin are less used by the network.  The parts of the activation function that are used change across the network (the early and late layers use different parts of the function) and during training (the preactivation distributions shift over time).  These plots verify that the negative bump in this activation function is important since it is heavily utilized by the neural network, especially by the late layer during the later epochs of training.}
    \label{fig:pangaea:preactivation}
\end{figure}

==> chapters/pangaea/figures/repeated_results.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Original PANGAEA Run}\\
        $\alpha x - \beta \log(\sigma(\gamma x))$ & 
        $71.01 {\scriptscriptstyle \pm 0.64}$ \\
        $\alpha x - \log(\sigma(\beta x))$ & 
        $70.30 {\scriptscriptstyle \pm 0.58}$ \\
        $\max\{\textrm{Swish}(x), 0\}$ & 
        $69.43 {\scriptscriptstyle \pm 0.69}$ \\
        \midrule
        
        \textbf{Additional PANGAEA Run 1} \\
        $\max \{ \min\{ \alpha \cdot x , \textrm{ELU}(x)\} , 0 \}$ & $70.53 {\scriptscriptstyle \pm 0.31}$\\ 
        $\alpha \cdot \max\left\{\beta \cdot \textrm{ReLU}\left(\frac{\textrm{Swish}(x)}{\gamma}\right), x\right\}$ & $70.52 {\scriptscriptstyle \pm 0.39}$\\
        $\max\{ \textrm{ReLU}(\textrm{Swish}(\alpha \cdot x)), \beta \cdot x\}$ & $70.44 {\scriptscriptstyle \pm 0.44}$\\
        \midrule
        
        \textbf{Additional PANGAEA Run 2} \\
        $\max\{ \textrm{Swish}(\alpha \cdot x), x \}$ & $\bm{71.03} {\scriptscriptstyle \pm 0.40}$\\
        $\max\{ \textrm{Swish}(x), \textrm{arcsinh}(\alpha \cdot \beta \cdot x)\}$ & $70.52 {\scriptscriptstyle \pm 0.35}$\\ 
        $\max\{ \textrm{Swish}(x), \textrm{arcsinh}(\alpha \cdot x)\}$ & $70.41 {\scriptscriptstyle \pm 0.38}$\\
        \midrule
        ReLU & $69.64 {\scriptscriptstyle \pm 0.65}$\\
        \bottomrule
    \end{tabular}
    \caption{Activation functions discovered with repeated independent PANGAEA runs on ResNet-v1-56.  Results shown are the CIFAR-100 test set accuracy aggregated over ten runs, shown as mean $\pm$ sample standard deviation.  Repeating PANGAEA from scratch produces activation functions that have different functional forms and yet achieve similarly high accuracy.}
    \label{tab:pangaea:repeated_results}
\end{table}


==> chapters/pangaea/figures/results_old.tex <==

\begin{table*}
    \centering
    \caption{CIFAR-100 test set accuracy shown as a median of ten runs, with mean $\pm$ sample standard deviation in parenthesis.  Asterisks indicate a statistically significant improvement in mean accuracy over ReLU, with * if $p \leq 0.05$, ** if $p \leq 0.01$, and *** if $p \leq 0.001$;  $p$-values are from one-tailed Welch's $t$-tests.  The top accuracy for each architecture is in bold, and results that are not statistically different from the top accuracy are also in bold.  Baseline activation function details are in \ref{ap:baseline}.\newline
    }
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{llll} \toprule
    & \textbf{WRN-10-4} & \textbf{ResNet-v1-56} & \textbf{ResNet-v2-56} \\ \midrule

    \textbf{Specialized for WRN-10-4}\\
    $\log(\sigma(\alpha x)) \cdot \textrm{arcsinh}(x)$ & 
    \cellcolor{black!5} \boldsymbol{$73.23$} {\scriptsize $(73.16 \pm 0.41)$ ***} &
    $11.15$ {\scriptsize $(19.34 \pm 20.14)$} &
    \boldsymbol{$72.05$} {\scriptsize $(64.30 \pm 21.32)$} \\
    
    $\log(\sigma(\alpha x)) \cdot \beta \textrm{arcsinh}(x)$ & 
    \cellcolor{black!5} \boldsymbol{$73.22$} {\scriptsize $(73.20 \pm 0.37)$ ***} &
    $05.78$ {\scriptsize $(18.63 \pm 21.04)$} &
    $55.40$ {\scriptsize $(45.88 \pm 30.70)$} \\
    
    $-\textrm{Swish}(\textrm{Swish}(\alpha x))$ & 
    \cellcolor{black!5} $72.38$ {\scriptsize $(72.49 \pm 0.55)$ ***} &
    $59.61$ {\scriptsize $(58.86 \pm 2.88)$} &
    $74.70$ {\scriptsize $(74.71 \pm 0.20)$ *} \\ 
    \midrule 

    \textbf{Specialized for ResNet-v1-56}\\
    $\alpha x - \beta \log(\sigma(\gamma x))$ & 
    $70.35$ {\scriptsize $(70.28 \pm 0.37)$} &
    \cellcolor{black!5} \boldsymbol{$70.82$} {\scriptsize $(71.01 \pm 0.64)$ ***} &
    $74.41$ {\scriptsize $(74.35 \pm 0.45)$} \\
    
    $\alpha x - \log(\sigma(\beta x))$ & 
    $70.62$ {\scriptsize $(70.47 \pm 0.53)$} &
    \cellcolor{black!5} $70.30$ {\scriptsize $(70.30 \pm 0.58)$ *} &
    $74.73$ {\scriptsize $(74.70 \pm 0.23)$ *} \\
    
    $\max\{\textrm{Swish}(x), 0\}$ & 
    $71.96$ {\scriptsize $(72.10 \pm 0.33)$ **} &
    \cellcolor{black!5} $69.46$ {\scriptsize $(69.43 \pm 0.69)$} &
    $74.97$ {\scriptsize $(74.97 \pm 0.25)$ **} \\
    \midrule 
    
    \textbf{Specialized for ResNet-v2-56}\\
    $\textrm{Softplus}(\textrm{ELU}(x))$ & 
    $71.51$ {\scriptsize $(71.36 \pm 0.34)$} &
    $69.94$ {\scriptsize $(69.96 \pm 0.39)$} &
    \cellcolor{black!5} \boldsymbol{$75.60$} {\scriptsize $(75.61 \pm 0.42)$ ***} \\
    
    $\min\{\log(\sigma(x)), \alpha \log(\sigma(\beta x))\}$ & 
    $72.05$ {\scriptsize $(72.04 \pm 0.34)$ **} &
    $69.63$ {\scriptsize $(69.56 \pm 0.48)$} &
    \cellcolor{black!5} $75.20$ {\scriptsize $(75.19 \pm 0.39)$ ***} \\
    
    $\textrm{SELU}(\textrm{Swish}(x))$ & 
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    \cellcolor{black!5} $75.06$ {\scriptsize $(75.02 \pm 0.35)$ **} \\
    \midrule 
    
    \textbf{General Activation Functions}\\
    $\max\{\textrm{Swish}(x), \alpha \log (\sigma (\textrm{ReLU}(x)))\}$ & 
     $72.50$ {\scriptsize $(72.54 \pm 0.26)$ ***} &
     $69.97$ {\scriptsize $(69.91 \pm 0.37)$} &
     $75.21$ {\scriptsize $(75.20 \pm 0.41)$ ***} \\
    
    $\min\{\textrm{Swish}(x), \alpha \textrm{ELU}(\textrm{ReLU}(\beta x))\}$ & 
     $72.44$ {\scriptsize $(72.39 \pm 0.29)$ ***} &
     $69.90$ {\scriptsize $(69.82 \pm 0.40)$} &
     $75.20$ {\scriptsize $(75.27 \pm 0.38)$ ***} \\
    
    $\log(\sigma(x))$ & 
     $72.38$ {\scriptsize $(72.33 \pm 0.32)$ ***} &
     $69.49$ {\scriptsize $(69.58 \pm 0.35)$} &
     \boldsymbol{$75.45$} {\scriptsize $(75.53 \pm 0.37)$ ***} \\
    \midrule
    
    \textbf{Fixed Baseline Functions}\\
    $\textrm{ReLU}$ &
    $71.44$ {\scriptsize $(71.46 \pm 0.50)$} &
    $69.78$ {\scriptsize $(69.64 \pm 0.65)$} &
    $74.43$ {\scriptsize $(74.39 \pm 0.44)$} \\

    $\textrm{ELiSH}$ & 
     $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $75.16$ {\scriptsize $(75.20 \pm 0.31)$ ***} \\
    
    $\textrm{ELU}$ & 
     $72.41$ {\scriptsize $(72.30 \pm 0.32)$ ***} &
    $69.59$ {\scriptsize $(69.67 \pm 0.46)$} &
    $74.86$ {\scriptsize $(74.95 \pm 0.30)$ **} \\
    
    $\textrm{GELU}$ & 
     $72.00$ {\scriptsize $(71.95 \pm 0.35)$ *} &
    $70.16$ {\scriptsize $(70.19 \pm 0.40)$ *} &
    $74.84$ {\scriptsize $(74.86 \pm 0.33)$ **} \\
    
    $\textrm{HardSigmoid}$ & 
     $55.55$ {\scriptsize $(54.99 \pm 1.00)$} &
    $33.31$ {\scriptsize $(32.55 \pm 4.06)$} &
    $65.03$ {\scriptsize $(64.90 \pm 0.69)$} \\
    
    $\textrm{Leaky ReLU}$ & 
     $71.76$ {\scriptsize $(71.73 \pm 0.33)$} &
    $69.77$ {\scriptsize $(69.78 \pm 0.33)$} &
    $74.75$ {\scriptsize $(74.73 \pm 0.35)$ *} \\
    
    $\textrm{Mish}$ & 
     $72.02$ {\scriptsize $(71.95 \pm 0.41)$ *} &
    $70.03$ {\scriptsize $(69.88 \pm 0.54)$} &
    $75.33$ {\scriptsize $(75.32 \pm 0.29)$ ***} \\
    
    $\textrm{SELU}$ & 
     $70.55$ {\scriptsize $(70.53 \pm 0.42)$} &
    $68.51$ {\scriptsize $(68.52 \pm 0.29)$} &
    $73.86$ {\scriptsize $(73.79 \pm 0.36)$} \\
    
    $\textrm{sigmoid}$ & 
     $56.45$ {\scriptsize $(56.10 \pm 0.98)$} &
    $37.07$ {\scriptsize $(36.47 \pm 3.32)$} &
    $66.72$ {\scriptsize $(66.45 \pm 0.92)$} \\
    
    $\textrm{Softplus}$ & 
     $72.25$ {\scriptsize $(72.27 \pm 0.26)$ ***} &
    $69.71$ {\scriptsize $(69.71 \pm 0.36)$} &
    \boldsymbol{$75.47$} {\scriptsize $(75.46 \pm 0.52)$ ***} \\
    
    $\textrm{Softsign}$ & 
     $56.72$ {\scriptsize $(56.30 \pm 2.16)$} &
    $58.33$ {\scriptsize $(58.38 \pm 0.96)$} &
    $69.31$ {\scriptsize $(69.33 \pm 0.39)$} \\
    
    $\textrm{Swish}$ & 
     $72.27$ {\scriptsize $(72.26 \pm 0.28)$ ***} &
    $69.60$ {\scriptsize $(69.68 \pm 0.38)$} &
    $75.17$ {\scriptsize $(75.08 \pm 0.36)$ ***} \\
    
    $\textrm{tanh}$ & 
     $56.29$ {\scriptsize $(56.52 \pm 1.53)$} &
    $63.89$ {\scriptsize $(63.88 \pm 0.38)$} &
    $70.53$ {\scriptsize $(70.44 \pm 0.40)$} \\
    \midrule
    
    \textbf{Parametric Baseline Functions}\\
    % Moved to appendix
    % $\alpha \textrm{ReLU}(\beta x)$ & 
    % $72.01$ {\scriptsize $(71.96 \pm 0.31)$ **} &
    % $68.91$ {\scriptsize $(68.93 \pm 0.22)$} &
    % $73.60$ {\scriptsize $(73.52 \pm 0.37)$} \\
    
    % $\alpha \textrm{ELiSH}(\beta x)$ & 
    % $01.00$ {\scriptsize $(01.00 \pm 0.00)$}&
    % $01.00$ {\scriptsize $(01.00 \pm 0.00)$}&
    % $73.95$ {\scriptsize $(73.94 \pm 0.33)$}\\
    
    % $\alpha \textrm{ELU}(\beta x)$ & 
    % $71.96$ {\scriptsize $(71.98 \pm 0.24)$ **} &
    % $68.91$ {\scriptsize $(69.06 \pm 0.37)$} &
    % $74.03$ {\scriptsize $(73.97 \pm 0.45)$} \\
    
    % $\alpha \textrm{GELU}(\beta x)$ & 
    % $71.86$ {\scriptsize $(71.96 \pm 0.34)$ **} &
    % $69.35$ {\scriptsize $(69.39 \pm 0.35)$} & 
    % $73.77$ {\scriptsize $(73.83 \pm 0.24)$} \\
    
    % $\alpha \textrm{HardSigmoid}(\beta x)$ & 
    % $66.74$ {\scriptsize $(66.70 \pm 0.64)$} &
    % $33.47$ {\scriptsize $(34.33 \pm 6.53)$} &
    % $65.09$ {\scriptsize $(65.10 \pm 0.40)$} \\ 
    
    % $\alpha \textrm{Leaky ReLU}(\beta x)$ & 
    % $71.70$ {\scriptsize $(71.74 \pm 0.39)$} &
    % $69.18$ {\scriptsize $(69.11 \pm 0.47)$} &
    % $73.53$ {\scriptsize $(73.44 \pm 0.29)$} \\ 
    
    % $\alpha \textrm{Mish}(\beta x)$ & 
    % $72.02$ {\scriptsize $(72.11 \pm 0.31)$ **} &
    % $69.66$ {\scriptsize $(69.51 \pm 0.67)$} &
    % $73.72$ {\scriptsize $(73.72 \pm 0.32)$} \\
    
    % $\alpha \textrm{SELU}(\beta x)$ & 
    % $71.04$ {\scriptsize $(71.07 \pm 0.33)$} &
    % $68.06$ {\scriptsize $(68.05 \pm 0.39)$} &
    % $73.44$ {\scriptsize $(73.37 \pm 0.38)$} \\
    
    % $\alpha \textrm{sigmoid}(\beta x)$ & 
    % $67.16$ {\scriptsize $(66.98 \pm 0.66)$} &      
    % $43.72$ {\scriptsize $(44.40 \pm 2.62)$} &
    % $66.80$ {\scriptsize $(66.98 \pm 0.85)$} \\ 
    
    % $\alpha \textrm{Softplus}(\beta x)$ & 
    % $71.82$ {\scriptsize $(71.73 \pm 0.31)$} &
    % $68.84$ {\scriptsize $(68.84 \pm 0.30)$} &
    % $73.92$ {\scriptsize $(73.95 \pm 0.37)$} \\ 
    
    % $\alpha \textrm{Softsign}(\beta x)$ & 
    % $62.19$ {\scriptsize $(62.12 \pm 0.83)$} &
    % $01.00$ {\scriptsize $(9.18 \pm 13.75)$} &
    % $68.91$ {\scriptsize $(68.87 \pm 0.38)$} \\ 
    
    % $\alpha \textrm{Swish}(\beta x)$ & 
    % $72.36$ {\scriptsize $(72.26 \pm 0.29)$ ***} &
    % $69.25$ {\scriptsize $(69.25 \pm 0.28)$} &
    % $73.97$ {\scriptsize $(73.93 \pm 0.22)$} \\ 
    
    % $\alpha \textrm{tanh}(\beta x)$ & 
    % $63.72$ {\scriptsize $(63.55 \pm 0.56)$} &
    % $01.00$ {\scriptsize $(02.92 \pm 6.07)$} &
    % $69.61$ {\scriptsize $(69.55 \pm 0.62)$} \\ 
    
    $\textrm{PReLU}$ &
    $72.25$ {\scriptsize $(72.23 \pm 0.37)$ ***} &
    $69.67$ {\scriptsize $(69.77 \pm 0.40)$} &
    $74.99$ {\scriptsize $(75.10 \pm 0.53)$ **} \\

    $\textrm{PSwish} = x \cdot \sigma(\beta x)$ & 
    $72.46$ {\scriptsize $(72.40 \pm 0.31)$ ***} &
    $70.19$ {\scriptsize $(70.16 \pm 0.46)$ *} &
    \boldsymbol{$75.37$} {\scriptsize $(75.39 \pm 0.28)$ ***} \\
    \midrule
    
    \textbf{Learnable Baseline Functions}\\
    $\textrm{APL}$ &
    $72.91$ {\scriptsize $(72.88 \pm 0.32)$ ***} &
    \boldsymbol{$70.88$} {\scriptsize $(70.81 \pm 0.20)$ ***} &
    $74.94$ {\scriptsize $(75.02 \pm 0.28)$ ***} \\

    $\textrm{PAU}$ &
    $45.85$ {\scriptsize $(41.46 \pm 22.66)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(02.38 \pm 4.36)$} \\
    
    $\textrm{SPLASH}$ &
    $72.25$ {\scriptsize $(72.16 \pm 0.81)$ *} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $73.54$ {\scriptsize $(73.45 \pm 0.43)$} \\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2em}
    % \label{tab:results}
\end{table*}

==> chapters/pangaea/figures/saturation.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cc}
       $\textrm{tanh}(x)$ & $\alpha\textrm{tanh}(\beta x)$\\
        \includegraphics[clip, trim=0em 0em 0em 2em, width=0.45\linewidth]{chapters/pangaea/images/tanh.png} 
        & \includegraphics[clip, trim=0em 0em 0em 2em, width=0.45\linewidth]{chapters/pangaea/images/ptanh.png}\\
        \emph{(a)} & \emph{(b)}
    \end{tabular}
    \caption{Parametric activation functions are more resistant to vanishing gradients.  When training with the $\textrm{tanh}(x)$ activation function in \emph{(a)}, the preactivation distribution in the late layer moves to the saturated regime.  The gradients in this layer will be near zero.  In this training instance, the network achieved chance accuracy (10\%).  When training with the parametric activation function $\alpha \tanh(\beta x)$ in \emph{(b)}, the values $\alpha$ and $\beta$ are updated by gradient descent during backpropagation.  Since $\alpha$ and $\beta$ are different in different layers, each layer has a slightly different activation function.  In this case, the preactivations do not saturate, and the network achieves good accuracy, i.e.\ just shy of 80\%.}
    \label{fig:pangaea:saturation}
\end{figure}

==> chapters/pangaea/figures/scatter_hist.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/scatter_hist.pdf}
    \caption{Fitness (validation accuracy) and compute cost (runtime in hours) among all activation functions considered in two independent PANGAEA processes.  Each point represents a unique activation function.  The distribution of fitness and compute cost are shown in histograms on the top and right, respectively.  Both PANGAEA processes reliably discover many novel activation functions that outperform ReLU.}
    \label{fig:pangaea:scatter_hist}
\end{figure}

==> chapters/pangaea/sections/custom.tex <==

\section{Training with Custom Activation Functions}
\label{sec:pangaea:custom}

This section demonstrates how to implement different activation functions in a TensorFlow neural network.  For example, the code to create the All-CNN-C architecture with a custom activation function is:

{\scriptsize
\begin{verbatim}
def all_cnn_c(args):
    inputs = Input((32, 32, 3))
    x = Conv2D(96, kernel_size=3, strides=(1, 1), padding='same', kernel_regularizer=l2(0.001))(inputs)
    x = CustomActivation(args)(x)
    x = Conv2D(96, kernel_size=3, strides=(1, 1), padding='same', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Conv2D(96, kernel_size=3, strides=(2, 2), padding='same', kernel_regularizer=l2(0.001))(x)
    x = Dropout(0.5)(x)

    x = Conv2D(192, kernel_size=3, strides=(1, 1), padding='same', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Conv2D(192, kernel_size=3, strides=(1, 1), padding='same', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Conv2D(192, kernel_size=3, strides=(2, 2), padding='same', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Dropout(0.5)(x)

    x = Conv2D(192, kernel_size=3, strides=(1, 1), padding='same', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Conv2D(192, kernel_size=1, strides=(1, 1), padding='valid', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)
    x = Conv2D(10, kernel_size=1, strides=(1, 1), padding='valid', kernel_regularizer=l2(0.001))(x)
    x = CustomActivation(args)(x)

    x = GlobalAveragePooling2D()(x)
    x = Flatten()(x)
    outputs = Activation('softmax')(x)

    return Model(inputs=inputs, outputs=outputs)
\end{verbatim}}

Here, \texttt{CustomActivation()} is a wrapper that resolves to different activation functions depending on the \texttt{args} parameter.  After importing \texttt{from tensorflow.keras.layers import Activation}, built-in activation functions can be implemented as \texttt{Activation('relu')} or \texttt{Activation('tanh')}, for example.  Activation functions that are not built in and do not contain learnable parameters can be implemented with lambda functions.  For example, the Mish activation function can be implemented with \texttt{Activation(lambda x : x * tf.math.tanh(tf.keras.activations.softplus(x)))}.  Finally, activation functions with learnable parameters simply require subclassing a \texttt{Layer} object.  The code used to implement the PAU activation function is below; APL and SPLASH are implemented in a similar manner.

{\scriptsize
\begin{verbatim}
"""
Padé Activation Units: End-to-end Learning of Flexible Activation Functions in Deep Networks
https://arxiv.org/abs/1907.06732

PAU of degree (5, 4) initialized to approximate Leaky ReLU (0.01)
"""
import tensorflow as tf

from tensorflow.keras.layers import Layer
from tensorflow.keras.initializers import Constant

class PAU(Layer):
    def __init__(self, num_init=None, denom_init=None, param_shape='per-layer', **kwargs):
        super(PAU, self).__init__(**kwargs)
        self.num_init = num_init if num_init else [0.02979246, 0.61837738, 2.32335207, 3.05202660, 1.48548002, 0.25103717]
        self.denom_init = denom_init if denom_init else [1.14201226, 4.39322834, 0.87154450, 0.34720652]
        self.num_weights = []
        self.denom_weights = []
        self.param_shape = param_shape

    def build(self, input_shape):
        if self.param_shape == 'per-layer':
            param_shape = (1,)
        elif self.param_shape == 'per-channel':
            param_shape = list(input_shape[-1:])
        else:
            assert self.param_shape == 'per-neuron'
            param_shape = list(input_shape[1:])

        for i in range(6):
            self.num_weights.append(
                self.add_weight(
                    name=f'a{i}',
                    shape=param_shape,
                    initializer=Constant(self.num_init[i]),
                    trainable=True))
        for i in range(4):
            self.denom_weights.append(
                self.add_weight(
                    name=f'b{i+1}',
                    shape=param_shape,
                    initializer=Constant(self.denom_init[i]),
                    trainable=True))

    def call(self, inputs):
        num = tf.add_n([self.num_weights[i] * tf.math.pow(inputs, i) for i in range(6)])
        denom = 1 + tf.math.abs(tf.add_n([self.denom_weights[i] * tf.math.pow(inputs, i+1) for i in range(4)]))
        return num / denom

    def get_config(self):
        config = super(PAU, self).get_config()
        config.update({'num_init'    : self.num_init,
                       'denom_init'  : self.denom_init,
                       'param_shape' : self.param_shape})
        return config

\end{verbatim}
}


==> chapters/pangaea/sections/implementation.tex <==
\section{Implementation and Compute Requirements}
\label{sec:pangaea:implementation}

High-performance computing in two clusters is utilized for the experiments. One cluster uses HTCondor \citep{thain2005distributed} for scheduling jobs, while the other uses the Slurm workload manager.  Training is executed on GeForce GTX 1080 and 1080 Ti GPUs on both clusters.  When a job begins executing, a parent activation function is selected by sampling $S=16$ functions from the $P=64$ most recently evaluated activation functions.  This is a minor difference from the original regularized evolution \citep{real2019regularized}, which is based on a strict sliding window of size $P$.  This approach may give extra influence to some activation functions, depending on how quickly or slowly jobs are executed in each of the clusters.  In practice the method is highly effective; it allows evolution to progress quickly by taking advantage of extra compute when demand on the clusters is low. 

It is difficult to know ahead of time how computationally expensive the evolutionary search will be.  Some activation functions immediately result in an undefined loss, causing training to end.  In that case only a few seconds have been spent and another activation function can immediately be evaluated.  Other activation functions train successfully, but their complicated expressions result in longer-than-usual training times.  
%In these experiments, evolution for WRN-10-4 took 2,314 GPU hours, evolution for ResNet-v1-56 took 1,594 GPU hours, and evolution for ResNet-v2-56 took 2,175 GPU hours.  These numbers do not include costs for reranking and repeated runs in the final experiments.  
Although substantial, the computational cost is negligible compared to the cost in human labor in designing activation functions.  Evolution of parametric activation functions requires minimal manual setup and delivers automatic improvements in accuracy.


==> chapters/pangaea/sections/training_details.tex <==
\section{Training Details \todo}
\label{sec:pangaea:details}

\subsection{Wide Residual Network (WRN-10-4)}

When measuring final performance after evolution, the standard WRN setup is used; all ReLU activations in WRN-10-4 are replaced with the evolved activation function, but no other changes to the architecture are made.  The network is optimized using stochastic gradient descent with Nesterov momentum 0.9.  The network is trained for 200 epochs; the initial learning rate is 0.1, and it is decreased by a factor of 0.2 after epochs 60, 120, and 160.  Dropout probability is set to 0.3, and L2 regularization of 0.0005 is applied to the weights.  Data augmentation includes featurewise center, featurewise standard deviation normalization, horizontal flip, and random $32 \times 32$ crops of images padded with four pixels on all sides.  This setup was chosen to mirror the original WRN setup \citep{zagoruyko2016wide} as closely as possible.

During evolution of activation functions, the training is compressed to save time. The network is trained for only 100 epochs; the learning rate begins at 0.1 and is decreased by a factor of 0.2 after epochs 30, 60, and 80.  Empirically, the accuracy achieved by this shorter schedule is sufficient to guide evolution; the computational cost saved by halving the time required to evaluate an activation function can then be used to search for additional activation functions.

\subsection{Residual Network (ResNet-v1-56)}



As with WRN-10-4, when measuring final performance with ResNet-v1-56, the only change to the architecture is replacing the ReLU activations with an evolved activation function.  The network is optimized with stochastic gradient descent and momentum 0.9.  Dropout is not used, and L2 regularization of 0.0001 is applied to the weights.  In the original ResNet experiments \citep{he2016deep}, an initial learning rate of 0.01 was used for 400 iterations before increasing it to 0.1, and further decreasing it by a factor of 0.1 after 32K and 48K iterations.  An iteration represents a single forward and backward pass over one training batch, while an epoch consists of training over the entire training dataset.  In this paper, the learning rate schedule is implemented by beginning with a learning rate of 0.01 for one epoch, increasing it to 0.1, and then decreasing it by a factor of 0.1 after epochs 91 and 137.  (For example, (48K iterations / 45K training images) * batch size of 128 $\approx$ 137.)  The network is trained for 200 epochs in total.  Data augmentation includes a random horizontal flip and random $32 \times 32$ crops of images padded with four pixels on all sides, as in the original setup \citep{he2016deep}.

When evolving activation functions for ResNet-v1-56, the learning rate schedule is again compressed.  The network is trained for 100 epochs; the initial warmup learning rate of 0.01 still lasts one epoch, the learning rate increases to 0.1, and then decreases by a factor of 0.1 after epochs 46 and 68.  When evolving activation functions, their relative performance is more important than the absolute accuracies they achieve.  The shorter training schedule is therefore a cost-efficient way of discovering high-performing activation functions.

\subsection{Preactivation Residual Network (ResNet-v2-56)}

The full training setup, data augmentation, and compressed learning rate schedule used during evolution for ResNet-v2-56 are all identical to those for ResNet-v1-56 with one exception: with ResNet-v2-56, it is not necessary to warm up training with an initial learning rate of 0.01 \citep{he2016identity}, so this step is skipped.

\subsection{All-CNN-C} When measuring final performance with All-CNN-C, the ReLU activation function is replaced with an evolved one, but the setup otherwise mirrors that of \citet{springenberg2015striving} as closely as possible.  The network is optimized with stochastic gradient descent and momentum 0.9.  Dropout probability is 0.5, and L2 regularization of 0.001 is applied to the weights.  The data augmentation involves featurewise centering and normalizing, random horizontal flips, and random $32 \times 32$ crops of images padded with five pixels on all sides.  The initial learning rate is set to 0.01, and it is decreased by a factor of 0.1 after epochs 200, 250, and 300.  The network is trained for 350 epochs in total.

During evolution of activation functions, the same training setup was used.  It is not necessary to compress the learning rate schedule as was done with the residual networks because All-CNN-C trains more quickly.

\subsection{CIFAR-10} As with CIFAR-100, a balanced validation set was created for CIFAR-10 by randomly selecting 500 images from each class, resulting in a training/validation/test split of 45K/5K/10K images.

